The Impact of Model Assumptions in Scalar-on-Image Regression

Complex statistical models such as scalar-on-image regression often require strong assumptions to overcome the issue of non-identifiability. While in theory it is well understood that model assumptions can strongly influence the results, this seems to be underappreciated, or played down, in practice. The article gives a systematic overview of the main approaches for scalar-on-image regression with a special focus on their assumptions. We categorize the assumptions and develop measures to quantify the degree to which they are met. The impact of model assumptions and the practical usage of the proposed measures are illustrated in a simulation study and in an application to neuroimaging data. The results show that different assumptions indeed lead to quite different estimates with similar predictive ability, raising the question of their interpretability. We give recommendations for making modeling and interpretation decisions in practice, based on the new measures and simulations using hypothetic coefficient images and the observed data.

==> captions/appBetaCI.tex <==
Coefficient image estimates for the application with pointwise $95\%$ confidence bands/credible intervals. Coloured pixels correspond to ``significant'' pixels, i.e.\ the confidence band/credible interval in this pixel does not contain zero. Note that some pixels too many might be flagged, as the confidence bands do not account for e.g.\  variable selection via cross-validation and are mostly calculated on a pointwise basis.  Note also the different scales for \textit{WPLS}, \textit{WNET} and \textit{GMRF}.

==> captions/appROIs.tex <==
Combining the results of the different methods in the application. Left: Agreement between ``significant'' regions. The value in each pixel corresponds to the number of models for which the  confidence band does not include zero for this pixel. 
Right: Correlation between the estimates within regions of interest defined on the basis of empirical confidence bands. See text for details.

==> captions/betaFuns.tex <==
Coefficient images $\beta$ used for the simulation. From left to right: 
\textit{bumpy}, \textit{pca} (based on the first $N = 250$ images in the dataset), \textit{smooth} and \textit{sparse}. Note the individual scale for each image.

==> captions/estErr_250_SNR_4.tex <==
Relative estimation errors for $N = 250$ observations and $\SNR = 4$ over all $100$ simulation runs.  
Boxplots show the errors for all models except \textit{GMRF} depending on the true coefficient image.
Gray horizontal lines mark $1$, which corresponds to a constant coefficient image, having the average value of the true $\beta$ image.

==> captions/expAss.tex <==
Parametric assumptions for the considered models.

==> captions/imageCovariates.tex <==
The first three image covariates $x_1, x_2, x_3$ after demeaning.

==> captions/impAss.tex <==
Underlying model assumptions for the considered models.
The order of the models has been slightly rearranged with respect to the presentation in Section~\ref{sec:methods} according to their assumptions.

==> captions/predErr_250_SNR_4_.tex <==
Relative prediction errors for $N = 250$ observations and $\SNR = 4$ over all $100$ simulation runs.  
Boxplots show the errors for all models except \textit{GMRF} depending on the true coefficient image.
Gray horizontal lines mark $1$, which corresponds to the simple intercept model.

==> captions/projBeta.tex <==
Values of $m_\text{Projection}$ for the different coefficient images depending on the basis functions.

==> captions/simBetaCorr250_SNR_4.tex <==
Median correlation between the true coefficient images and the estimates for $N = 250$ observations and $\SNR = 4$ over all $100$ simulation runs. The figures show the median  correlation of the vectorized images depending on the true images and the models.

==> captions/simExplicitAss250_SNR_4.tex <==
Measures for parametric model assumptions in the simulation for $N = 250$ observations and $\SNR = 4$ over all $100$ simulation runs. Boxplots show the measures for the different coefficient images depending on the model. All values on log-scale.

==> captions/simImplicitAss250_SNR_4.tex <==
Measures for underlying model assumptions in the simulation for $N = 250$  observations and $\SNR = 4$ over all $100$ simulation runs. Boxplots show the measures for the different models depending on the true coefficient image. All values on log-scale. Gray horizontal lines correspond to the values for the true coefficient images.
